Mechanised operational semantics of Rowhammer

Rowhammer is a hardware vulnerability in dynamic random-access memory (DRAM) in which repeated accesses to aggressor rows can induce bit-flips in victim rows. This phenomenon violates a core assumption of conventional programming language semantics: reading or writing one memory location does not modify others. Despite the security importance of this phenomenon, there is no formal framework connecting Rowhammer faults with program behaviour. We present a probabilistic small-step operational semantics for an idealised imperative language subject to Rowhammer-style faults. The semantics abstracts from DRAM internals and semiconductor physics. A general probabilistic fault model parameterises the semantics, representing Rowhammer-style faults by assigning probabilities to bit-flips during read or write operations. The resulting distributions are propagated through programs using the standard monadic structure of probabilistic computation. As a case study, we formalise a well-known defence that places program variables sufficiently far apart in physical memory that an access to one variable cannot disturb another. We prove a distribution-independent semantic collapse theorem: for every finite execution, including prefixes of terminating and non-terminating executions, the protected projection of the probabilistic Rowhammer semantics is the Dirac distribution of the corresponding Rowhammer-free execution. We develop an observation-parametric account of secure information flow. Non-interference is expressed as a hyperproperty comparing the distributions of low observations from low-equivalent initial memories. Consequently, physical separation preserves non-interference for every admissible fault model, while every Rowhammer non-interference violation reflects a violation already present in the Rowhammer-free semantics. The development is fully mechanised in Lean using mathlib.

==> generated/DivergencePreservation.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Goal.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
def DivergencePreservation : Prop :=
  ∀ (sep : SeparationModel) (f : ProbRHFlip sep),
    HasProbFlipFrame sep f →
    ∀ (br : Nat) (locs : LocSet),
      sep.isSafe br locs →
      ∀ (p : Prog), p.WellFormed locs →
        ∀ (m : Memory), Diverges p m →
          ∀ (n : Nat),
            ∀ c ∈ (runRH sep f br locs n (p, m)).support,
              c.1 ≠ Prog.skip
\end{lstlisting}


==> generated/HasProbFlipFrame.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Fault.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
class HasProbFlipFrame (sep : SeparationModel) (f : ProbRHFlip sep) : Prop where
  outside_unchanged : ∀ (S : LocSet) (m m' : Memory) (x : Loc),
    m' ∈ (f S m).support → x ∉ S → m' x = m x
\end{lstlisting}


==> generated/NoFaultEmbedding.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Goal.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
def NoFaultEmbedding : Prop :=
  ∀ (sep : SeparationModel) (br : Nat) (locs : LocSet)
    (P : Prog) (m : Memory),
    stepRHHat sep (noFlip sep) br locs P m
      = Dist.dirac (stepDHat P m)
\end{lstlisting}


==> generated/PhysicalSeparationSound.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Goal.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
def PhysicalSeparationSound : Prop :=
  ∀ (sep : SeparationModel) (f : ProbRHFlip sep),
    HasProbFlipFrame sep f →
    ∀ (br : Nat) (locs : LocSet),
      sep.isSafe br locs →
      ∀ (p : Prog), p.WellFormed locs →
        ∀ (m : Memory) (n : Nat),
          Dist.mapD (protView locs)
              (runRHTrace sep f br locs n (p, m))
            = Dist.dirac (protView locs (runDTrace n (p, m)))
\end{lstlisting}


==> generated/ProbRHFlip.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Fault.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
abbrev ProbRHFlip (_sep : SeparationModel) :=
  LocSet → Memory → Dist Memory
\end{lstlisting}


==> generated/SeparationModel.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Fault.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
structure SeparationModel where
  adj : Nat → LocSet → Loc → LocSet
  isSafe : Nat → LocSet → Prop
  /-- Safe layouts: the victim set of an access to a protected row is
      disjoint from the protected set. -/
  safe_disjoint : ∀ {br : Nat} {locs : LocSet} {x : Loc},
    isSafe br locs → x ∈ locs → ∀ y ∈ locs, y ∉ adj br locs x
\end{lstlisting}


==> generated/TerminationCorrespondence.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Goal.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
def TerminationCorrespondence : Prop :=
  ∀ (sep : SeparationModel) (f : ProbRHFlip sep),
    HasProbFlipFrame sep f →
    ∀ (br : Nat) (locs : LocSet),
      sep.isSafe br locs →
      ∀ (p : Prog), p.WellFormed locs →
        ∀ (m m' : Memory) (s : List Access),
          PTrace (p, m) s (Prog.skip, m') →
          ∀ c ∈ (runRH sep f br locs s.length (p, m)).support,
            c.1 = Prog.skip ∧ ∀ x ∈ locs, c.2 x = m' x
\end{lstlisting}


==> generated/WellFormed.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Basic.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
def WellFormed (locs : LocSet) : Prog → Prop
  | skip => True
  | assign x e => x ∈ locs ∧ e.WellFormed locs
  | seq p q => p.WellFormed locs ∧ q.WellFormed locs
  | ite b p q => b.WellFormed locs ∧ p.WellFormed locs ∧ q.WellFormed locs
  | whileDo b p => b.WellFormed locs ∧ p.WellFormed locs
\end{lstlisting}


==> generated/corruptAll.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Fault.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
noncomputable def corruptAll (sep : SeparationModel) : ProbRHFlip sep :=
  fun S m => dirac (fun x => if x ∈ S then m x + 1 else m x)
\end{lstlisting}


==> generated/pRHStep_iff_stepRHHat.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Agreement.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
theorem pRHStep_iff_stepRHHat {P : Prog} {m : Memory}
    (hP : P ≠ Prog.skip) {μ : Dist (Prog × Memory)} :
    PRHStep sep f br locs (P, m) μ ↔ stepRHHat sep f br locs P m = μ := by
  constructor
  · exact pRHStep_agree
  · rintro rfl
    exact stepRHHat_step P m hP
\end{lstlisting}


==> generated/physical_separation_sound.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Soundness.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
theorem physical_separation_sound : PhysicalSeparationSound := by
  intro sep f hframe br locs hsafe p hwf m n
  apply Dist.mapD_eq_dirac_of_support
  intro r hr
  have hsub : ∀ x ∈ locs, x ∈ locs := fun x hx => hx
  have hpres : ∀ x ∈ locs, ∀ (m₀ m' : Memory),
      m' ∈ (f (sep.adj br locs x) m₀).support → ∀ ℓ, ℓ ∈ locs → m' ℓ = m₀ ℓ :=
    fun x hx m₀ m' hm' ℓ hℓ =>
      hframe.outside_unchanged _ m₀ m' ℓ hm' (sep.safe_disjoint hsafe hx ℓ hℓ)
  obtain ⟨h1, h2, h3⟩ :=
    runRHTrace_protected (keep := (· ∈ locs)) hsub hpres n hwf
      (AgreeP.refl _ m) r hr
  simp only [protView, Prod.mk.injEq]
  refine ⟨h1, ?_, ?_⟩
  · funext x
    exact h2 x.1 x.2
  · rw [h3]
\end{lstlisting}


==> generated/protView.tex <==
% AUTO-GENERATED from lean/SemanticCollapse/Goal.lean by lean/scripts/extract_snippets.sh — do not edit.
\begin{lstlisting}[language=Lean]
def protView (locs : LocSet) :
    (Prog × Memory) × List Access →
      Prog × ({x : Loc // x ∈ locs} → Val) × List Access :=
  fun r => (r.1.1, fun x => r.1.2 x.1, accessTrace r.2)
\end{lstlisting}

